Exploring Missing Modality in Multimodal Egocentric Datasets

Multimodal video understanding is crucial for analyzing egocentric videos, where integrating multiple sensory signals significantly enhances action recognition and moment localization. However, practical applications often grapple with incomplete modalities due to factors like privacy concerns, efficiency demands, or hardware malfunctions. Addressing this, our study delves into the impact of missing modalities on egocentric action recognition, particularly within transformer-based models. We introduce a novel concept -Missing Modality Token (MMT)-to maintain performance even when modalities are absent, a strategy that proves effective in the Ego4D, Epic-Kitchens, and Epic-Sounds datasets. Our method mitigates the performance loss, reducing it from its original $\sim 30\%$ drop to only $\sim 10\%$ when half of the test set is modal-incomplete. Through extensive experimentation, we demonstrate the adaptability of MMT to different training scenarios and its superiority in handling missing modalities compared to current methods. Our research contributes a comprehensive analysis and an innovative approach, opening avenues for more resilient multimodal systems in real-world settings.

==> cvpr/preamble.tex <==
%
% --- inline annotations
%
\usepackage[dvipsnames]{xcolor}
\newcommand{\red}[1]{{\color{red}#1}}
\newcommand{\todo}[1]{{\color{red}#1}}
\newcommand{\TODO}[1]{\textbf{\color{red}[TODO: #1]}}
\usepackage{graphicx} % Required for inserting images
\usepackage{color}
\usepackage{tabularray}
\usepackage{multirow}
\usepackage{algpseudocode}
\usepackage{array}
\usepackage{tabularx}
\usepackage{algorithm}
% \usepackage{float}
\usepackage{stfloats}
\usepackage{pifont}
\definecolor{stratOne}{HTML}{895259}
\definecolor{stratTwo}{HTML}{204d4f}
% --- disable by uncommenting  
% \renewcommand{\TODO}[1]{}
% \renewcommand{\todo}[1]{#1}
%% comment all before submission
\newcommand{\MRnote}[1]{{\color{violet}{\bf MR: }#1}} % teal
\newcommand{\MR}[1]{{\color{violet}#1}} % cyan
\newcommand{\APnote}[1]{{\color{cyan}{\bf AP: }#1}} % teal
\newcommand{\AP}[1]{{\color{cyan}#1}} % cyan
\newcommand{\HA}[1]{{\color{blue}{\bf HA: }#1}} % teal
%% uncomment all before submission
\renewcommand{\HA}[1]{{}}
% \renewcommand{\MRnote}[1]{{\color{violet}}} % violet
% \renewcommand{\MR}[1]{{\color{black}#1}} % violet
% \renewcommand{\APnote}[1]{{\color{violet}}} % violet
% \renewcommand{\AP}[1]{{\color{black}#1}} % violet

==> figures/ek-ego4d-p-ablation.tex <==
\begin{figure}[t!]
\begin{center}
\includegraphics[width=\linewidth]{images/coverage_EK_STA.pdf}
\end{center}
\small
\vspace{-5pt}
\caption{\textbf{ Modality drop probability $p$ \vs accuracy for Epic-Kitchens and Ego4D-AR}. For both datasets, using smaller $p = 25\%$ provides robustness to missing modality, while still preserving the optimal performance on modal-complete data ($r_{test} = 0\%$).} 
\label{fig:ek-ego4d-p-ablation}
\vspace{-10pt}
\end{figure}


==> figures/fusion_layers_2.tex <==
\begin{figure*}
\captionsetup[subfloat]{}
\centering
\begin{subfigure}[b]{\textwidth}
%   \centering
\includegraphics[width=\linewidth]{images/Epic-Sounds.pdf}
  \caption{Epic-Sounds}
  \label{subfig:fusion_es}
\end{subfigure}%
% \hfill

\begin{subfigure}[b]{\textwidth}
%   \centering
\includegraphics[width=\linewidth]{images/Epic-Kitchens.pdf}
  \caption{Epic-Kitchens}
  \label{subfig:fusion_ek}
\end{subfigure}
\caption{\textbf{Performance \vs Bottleneck fusion layer} inference with complete and missing inputs. \textbf{Left}: the models trained with complete inputs only. \textbf{Right}: the models trained with the missing modality tokens.}

\label{figure:fusion}
\end{figure*}

% \begin{figure*}[t!]
%  \captionsetup[subfloat]{font=scriptsize,labelfont=scriptsize}
% \begin{center}
% \includegraphics[width=\linewidth]{figures/Epic-Kitchens.png}
% \end{center}
% \small

% \caption{\textbf{} }
% % \vspace{-5mm}
% \label{figure:fusion_ek}
% \end{figure*}


==> tables/baseline_1_epic.tex <==



==> tables/baseline_1_oscc.tex <==
\begin{table}[]
    \centering
    \begin{tabular}{c|c}
         &  \\
         & 
    \end{tabular}
    \caption{Caption}
    \label{tab:my_label}
\end{table}

==> tables/intro-kitchen.tex <==
\begin{table}[ht!]
\setlength\tabcolsep{3pt}
    \centering
    \small
\begin{tabular}{c|c|c|c|c|c|c}
\toprule
\multicolumn{2}{c|}{\textbf{train}}                & \multicolumn{2}{c|}{\textbf{val}}                  & \multirow{2}{1.2cm}{\textbf{Missing modality}}                & \multicolumn{2}{c}{\textbf{Accuracy}} \\
% \hline
\textbf{Video} & \textbf{Audio} & \textbf{Video} & \textbf{Audio} & \textbf{} & \textbf{noun}          & \textbf{verb}         \\

\hline
0\%                     & 100\%                   & 0\%                     & 100\%                   & none                      & 17.87\%       & 40.05\%      \\
\hline
\multirow{3}{*}{100\%}  & \multirow{3}{*}{0\%}    & 100\%                   & \multirow{3}{*}{0\%}    & \multirow{3}{*}{video}    & 43.03\%       & 63.22\%      \\
                        &                         & 50\%                    &                         &                           & 21.34\%       & 32.76\%      \\
                        &                         & 25\%                    &                         &                           & 10.87\%       & 17.88\%    \\
                        \hline
\multirow{3}{*}{100\%}  & \multirow{3}{*}{100\%}  & 100\%                   & \multirow{3}{*}{100\%}  & \multirow{3}{*}{video}    & 42.40\%       & 63.93\%      \\
                        &                         & 50\%                    &                         &                           & 27.54\%       & 46.78\%      \\
                        &                         & 25\%                    &                         &                           & 20.19\%       & 37.86\%      \\
                        \bottomrule
\end{tabular}
  \caption{Epic-Kitchens}
  \label{table1:intro-kitchen}

\end{table}

==> tables/intro-sound.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[h]
\setlength\tabcolsep{3pt}
    \centering
    \small
\begin{tabular}{c|c|c|c|c|c}
\toprule
\multicolumn{2}{c|}{\textbf{train}}                & \multicolumn{2}{c|}{\textbf{val}}                  & \multirow{2}{1.2cm}{\textbf{Missing modality}}                & \multirow{2}{*}{\textbf{Accuracy} } \\ 
% \hline
\textbf{Video} & \textbf{Audio} & \textbf{Video} & \textbf{Audio} &  &    \\

                        \hline
100\%                   & 0\%                  & 100\%                   & 0\%                     & none                      & 41.41\%              \\
\hline
\multirow{3}{*}{0\%}    & \multirow{3}{*}{100\%}  & \multirow{3}{*}{0\%}    & 100\%                   & \multirow{3}{*}{audio}    & 44.24\%              \\
                        &                         &                         & 50\%                    &                           & 23.35\%              \\
                        &                         &                         & 25\%                    &                           & 12.57\%     \\
                        \hline
\multirow{3}{*}{100\%}  & \multirow{3}{*}{100\%}  & \multirow{3}{*}{100\%}  & 100\%                   & \multirow{3}{*}{audio}    & 55.15\%              \\
                        &                         &                         & 50\%                    &                           & 37.05\%              \\
                        &                         &                         & 25\%                    &                           & 28.25\%              \\
                        \bottomrule
\end{tabular}
    \caption{Epic Sounds}
      \label{table1:intro-sound}
\end{table}
